CHiQPM: Calibrated Hierarchical Interpretable Image Classification

Globally interpretable models are a promising approach for trustworthy AI in safety-critical domains. Alongside global explanations, detailed local explanations are a crucial complement to effectively support human experts during inference. This work proposes the Calibrated Hierarchical QPM (CHiQPM) which offers uniquely comprehensive global and local interpretability, paving the way for human-AI complementarity. CHiQPM achieves superior global interpretability by contrastively explaining the majority of classes and offers novel hierarchical explanations that are more similar to how humans reason and can be traversed to offer a built-in interpretable Conformal prediction (CP) method. Our comprehensive evaluation shows that CHiQPM achieves state-of-the-art accuracy as a point predictor, maintaining 99% accuracy of non-interpretable models. This demonstrates a substantial improvement, where interpretability is incorporated without sacrificing overall accuracy. Furthermore, its calibrated set prediction is competitively efficient to other CP methods, while providing interpretable predictions of coherent sets along its hierarchical explanation.

==> secs/SidewaysTables.tex <==
\begin{sidewaystable}[htbp]
%\resizebox{\linewidth}{!}{
  \centering

    \caption{
  \accmetricstablestart{\resnet{}}
  \cref{fig:dimVar} shows the increasing gap when further raising compactness. 
  \boldnessstatement
  %Comparison on typical metrics for prototype-based methods with \resnet{} as backbone: \gls{NewlayerName} shows increased accuracy with increased compactness. 
  %\boldnessstatement
  %The * indicates reported values which could not be reproduced.
  }
  \label{stab:aCCproto-table}
  \begin{tabular}{lcccccccccccc}
    \toprule
    Method &  \multicolumn{4}{c}{Accuracy \arrowUp} &
    \multicolumn{4}{c}{Total Features\arrowDown} & \multicolumn{4}{c}{Features / Class\arrowDown} \\
  & CUB& CARS & TRAVEL & IMGNET & CUB& CARS & TRAVEL & IMGNET & CUB& CARS &TRAVEL & IMGNET
    \\
    \midrule
    Baseline \resnet{} & {86.6}$\pm$0.2 & {92.1}$\pm$0.1 & {59.5}$\pm$0.9 &76.1  & 2048 & 2048 &2048& 2048& 2048& 2048 &2048&2048\\
    \midrule
    \glmtable{} & {78.0}$\pm$0.4 & {86.8}$\pm$0.6 & {58.0}$\pm$1.2 & 58.0$\pm$0.0 & 809$\pm$8 & 807$\pm$10 & 781$\pm$6 & 1627$\pm$1 & \textbf{5}& \textbf{5} &\textbf{5}&\textbf{5} \\
    \pipnettable{} & 82.0$\pm$0.3 & 86.5$\pm$0.3 & 74.0$\pm$0.4  &-& 731$\pm$19 &669$\pm$13& 744$\pm$15  &-& 12 &11 & 6& - \\ % my machine: 59.0, 450, 3.095
    % big machine 2: 70.6, 861, 5.8, 3: 68.79, 5.57, 840 1: 70.9, 775, 5.3
    \protopooltable{} & 79.4$\pm$0.4  &87.5$\pm$0.2 & 38.1$\pm$1.9 &-& 202 & 195 &202& -  &202 & 195 & 202 & - \\ %82.5 for Naturalist
    \slddtable{}  & {84.5}$\pm$0.2 & {91.1}$\pm$0.1 & \underline{75.6}$\pm$0.2 & 72.7$\pm$0.0 & \textbf{50} & \textbf{50} &\textbf{50}& \textbf{50}& \textbf{5}& \textbf{5} &\textbf{5}&\textbf{5} \\
     \gls{NewlayerName}   & \underline{85.1}$\pm$0.3 & \underline{91.8}$\pm$0.3 & \textbf{75.7}$\pm$0.8& \underline{74.2}$\pm$0.0 & \textbf{50} & \textbf{50} &\textbf{50}& \textbf{50}& \textbf{5}& \textbf{5} &\textbf{5}&\textbf{5} \\
      \midrule
      \tabOurs & &  & {75.2}$\pm$0.6  & \textbf{74.5}$\pm$0.1 & \textbf{50} &\textbf{50}& \textbf{50}&\textbf{50}& 10 &10 &10 &10 \\
     
     % Imgs, 74,192, 74.07, 74.254
  % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.3}& \textbf{77.2} & -&202 &195& 202&-& \textbf{5} &\textbf{5} &\textbf{5} &- \\
    % $\gls{nperClass}=10$ (Ours)  & \textbf{85.7}$\pm$0.2 & \textbf{92.1}$\pm$0.1 & {75.2}$\pm$0.6  & \textbf{74.5}$\pm$0.1 & \textbf{50} &\textbf{50}& \textbf{50}&\textbf{50}& 10 &10 &10 &10 \\
    % \multicolumn{5}{c}{CARS} \\
    % \midrule
    % PIP-Net & 86.5 & 669 & 11  \\
    % ProtoPool & 88.9 & 195 & 195 \\
    \bottomrule
  \end{tabular}
%  }

  
\end{sidewaystable}
\begin{sidewaystable}[htbp]
%
  \centering
  \caption{
  \interpmetricstablestart{\resnet{}}}
 % test}
  \resizebox{\textwidth}{!}{
% %   %Comparison on Interpretability metrics with \resnet{} as backbone. Due to required annotations, \cubsim{} can only be computed for \travelingheader{} and \cubheader{}. \boldnessstatement}
%    \label{stab:Interpproto-table}
  \begin{tabular}{lcccccccccccccc}
    \toprule
    Method &  \multicolumn{4}{c}{\loc{5} \arrowUp} &
    \multicolumn{4}{c}{\generality{}\arrowUp} & \multicolumn{4}{c}{\contrastiveness{}\arrowUp} & \multicolumn{2}{c}{\cubsim{}\arrowUp} \\
   & CUB& CARS & TRAVEL & IMGNET & CUB& CARS & TRAVEL & IMGNET & CUB& CARS &TRAVEL & IMGNET & CUB&TRAVEL
    \\
    \midrule
   Baseline \resnet{} & {57.7}$\pm$0.4 & {54.4}$\pm$0.3 & {59.9}$\pm$0.4 &37.1  & {98.0}$\pm$0.0 & {97.8}$\pm$0.0 & {98.0}$\pm$0.0&  99.4& {74.4}$\pm$0.1 & {75.1}$\pm$0.1 & {74.4}$\pm$0.1&71.6 &  {34.0}$\pm$0.3 &  {32.1}$\pm$0.2 \\
  \midrule
  \glmtable{}  & {55.4}$\pm$0.5 & {51.8}$\pm$0.3 & {56.0}$\pm$0.8&35.8$\pm$0.0   & \underline{97.8}$\pm$0.0 & \underline{97.6}$\pm$0.0 & \underline{97.8}$\pm$0.0 & \underline{99.4}$\pm$0.0  & {74.0}$\pm$0.1 & {74.5}$\pm$0.1 & {73.8}$\pm$0.1&71.7$\pm$0.0 & {2.5}$\pm$1.0 & {4.4}$\pm$2.8 \\
    \pipnettable{} & \textbf{99.2}$\pm$0.1 & \textbf{99.0}$\pm$0.1 & \textbf{98.7}$\pm$0.1&-  & 75.6$\pm$0.4 &62.9$\pm$0.1 & 73.4$\pm$0.1&-  & \textbf{99.6}$\pm$0.0 &\textbf{99.7}$\pm$0.0 & \textbf{99.7}$\pm$0.0&- & 6.7$\pm$0.9 & 6.9$\pm$1.3 \\ % my machine: 59.0, 450, 3.095
    % big machine 2: 70.6, 861, 5.8, 3: 68.79, 5.57, 840 1: 70.9, 775, 5.3
    \protopooltable{} & 24.5$\pm$0.8 &30.7$\pm$3.4& 31.5$\pm$1.6&-& 96.9$\pm$0.1 & 96.0$\pm$0.5 &95.5$\pm$0.1&- &76.7$\pm$1.0& 78.9$\pm$2.0 & 85.2$\pm$0.5&- & 13.9$\pm$0.9 & 7.6$\pm$2.5 \\
    \slddtable{}
     & {88.2}$\pm$0.2 & {88.6}$\pm$0.6 & {87.5}$\pm$0.4&\underline{64.7}$\pm$0.7 & {96.2}$\pm$0.1 & {95.5}$\pm$0.1 & {96.5}$\pm$0.1&{98.6}$\pm$0.0  & {87.3}$\pm$0.2 & {89.7}$\pm$0.3& {86.3}$\pm$0.2&\textbf{93.4}$\pm$0.1 &   {29.2}$\pm$4.0 &  {30.7}$\pm$3.1  \\
      \midrule
     \gls{NewlayerName} (Ours)  & {90.1}$\pm$0.3 & {89.6}$\pm$0.4 & {89.7}$\pm$0.2&{64.1}$\pm$0.7  & {97.0}$\pm$0.0 & {96.5}$\pm$0.0 & {97.2}$\pm$0.0 &{99.1}$\pm$0.0&   \underline{96.0}$\pm$0.4 & {97.7}$\pm$0.4& {94.0}$\pm$0.3&\underline{89.3}$\pm$0.1  &   \underline{47.9}$\pm$2.7 & \underline{54.3}$\pm$4.0\\
     $\gls{nperClass} = 10$ (Ours)  & \underline{95.8}$\pm$0.7 & \underline{96.6}$\pm$0.5 & \underline{95.1}$\pm$0.3 & \textbf{80.1}$\pm$0.9 & \textbf{98.1}$\pm$0.0 & \textbf{98.0}$\pm$0.1 & \textbf{98.1}$\pm$0.0 & \textbf{99.5}$\pm$0.0 & {95.9}$\pm$0.5 & \underline{98.6}$\pm$0.2&\underline{94.2}$\pm$0.3& 87.4$\pm$0.1 & \textbf{52.3}$\pm$1.6 &  \textbf{62.9}$\pm$2.8\\
    % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.2}& \textbf{78.4}  \\
    % \multicolumn{5}{c}{CARS} \\
    % \midrule
    % PIP-Net & 86.5 & 669 & 11  \\
    % ProtoPool & 88.9 & 195 & 195 \\
    \bottomrule
  \end{tabular}
  }
%\end{table*}
\end{sidewaystable}
\begin{sidewaystable}[htbp]
%\resizebox{\linewidth}{!}{
  \caption{
   \accmetricstablestart{Resnet34}
   \boldnessstatement
  %Comparison on typical metrics for prototype-based methods with Resnet34 as backbone: \gls{NewlayerName} shows increased accuracy with increased compactness. \boldnessstatement
  %The * indicates reported values which could not be reproduced.
  }
  \label{stab:r34aCCproto-table}
  \centering
  \begin{tabular}{lccccccccc}
    \toprule
    Method &  \multicolumn{3}{c}{Accuracy \arrowUp} &
    \multicolumn{3}{c}{Total Features\arrowDown} & \multicolumn{3}{c}{Features / Class\arrowDown} \\
   & CUB& CARS & TRAVEL   & CUB& CARS & TRAVEL  & CUB& CARS &TRAVEL 
    \\
    \midrule
    Baseline Resnet34 & 85.7$\pm$0.3 & 91.5$\pm$0.2 & 61.3$\pm$0.4   & 2048 & 2048 &2048&  2048& 2048 &2048\\
    \midrule
    \glmtable{} & {72.0}$\pm$1.0 & {82.0}$\pm$0.6 & {53.5}$\pm$0.8 & 442$\pm$5 & 453$\pm$6 & 443$\pm$6  & \textbf{5}& \textbf{5} &\textbf{5} \\
    \slddtable{} & \underline{83.2}$\pm$0.3 & {90.7}$\pm$0.3 & {74.0}$\pm$0.2  & \textbf{50} & \textbf{50} &\textbf{50}&  \textbf{5}& \textbf{5} &\textbf{5} \\
     \midrule
     \gls{NewlayerName} (Ours)  & {83.0}$\pm$0.2 & \underline{91.3}$\pm$0.0 & \underline{75.1}$\pm$0.3& \textbf{50} & \textbf{50} &\textbf{50}&  \textbf{5}& \textbf{5} &\textbf{5}\\ % Imgs, 74,192, 74.07, 74.254
   % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.3}& \textbf{77.2} & -&202 &195& 202&-& \textbf{5} &\textbf{5} &\textbf{5} &- \\
    $\gls{nperClass}=10$ (Ours) & \textbf{83.9}$\pm$0.1 & \textbf{91.7}$\pm$0.1 & \textbf{75.7}$\pm$0.6 & \textbf{50} &\textbf{50}& \textbf{50}& 10 &10 &10  \\
    % \multicolumn{5}{c}{CARS} \\
    % \midrule
    % PIP-Net & 86.5 & 669 & 11  \\
    % ProtoPool & 88.9 & 195 & 195 \\
    \bottomrule
  \end{tabular}
 % }

  
\end{sidewaystable}
\begin{sidewaystable}[htbp]
%\resizebox{\linewidth}{!}{
  \caption{
  \interpmetricstablestart{Resnet34}}
  %Comparison on Interpretability metrics with Resnet34 as backbone. Due to required annotations, \cubsim{} can only be computed for \travelingheader{} and \cubheader{}. \boldnessstatement}
  \label{stab:r34Interpproto-table}
  \centering
  \begin{tabular}{lccccccccccc}
    \toprule
    Method &  \multicolumn{3}{c}{\loc{5} \arrowUp} &
    \multicolumn{3}{c}{\generality{}\arrowUp} & \multicolumn{3}{c}{\contrastiveness{}\arrowUp} & \multicolumn{2}{c}{\cubsim{}\arrowUp} \\
  & CUB& CARS & TRAVEL   & CUB& CARS & TRAVEL   & CUB& CARS &TRAVEL   & CUB&TRAVEL
    \\
    \midrule
    Baseline Resnet34  & {62.1}$\pm$0.3 & {56.6}$\pm$0.4 & {64.1}$\pm$0.6  & {97.9}$\pm$0.0 & {97.7}$\pm$0.0 & {98.0}$\pm$0.0   & {76.4}$\pm$0.1 & {77.9}$\pm$0.2 & {76.0}$\pm$0.1   & {39.6}$\pm$0.2  & {36.0}$\pm$0.4 \\
    \midrule
    \glmtable{}  & {59.9}$\pm$0.4 & {55.3}$\pm$0.3 & {60.6}$\pm$0.4
  & \textbf{97.9}$\pm$0.0 & \underline{97.7}$\pm$0.0 & \underline{97.9}$\pm$0.0& {76.5}$\pm$0.0 & {77.8}$\pm$0.2 & {76.0}$\pm$0.1  &   {7.6}$\pm$2.2  & {9.4}$\pm$3.8 \\
    \slddtable{}
     & {90.1}$\pm$0.8 & {86.7}$\pm$2.5 & {87.3}$\pm$0.3    & {97.5}$\pm$0.0 & {97.6}$\pm$0.2 & {97.8}$\pm$0.0 & {86.0}$\pm$1.0 & {83.3}$\pm$4.6 & {82.0}$\pm$1.4  & {24.5}$\pm$2.7  & {29.4}$\pm$5.2 \\
      \midrule
     \gls{NewlayerName} (Ours)  & \underline{90.5}$\pm$0.5 & \underline{89.1}$\pm$1.1 & \underline{89.7}$\pm$0.7 & {97.5}$\pm$0.0 & {96.9}$\pm$0.1 & {97.6}$\pm$0.0  &   \underline{95.5}$\pm$0.2 & \underline{94.7}$\pm$1.1 & \underline{94.3}$\pm$0.5 & \underline{39.0}$\pm$2.9 & \underline{49.7}$\pm$4.7\\
     $\gls{nperClass} = 10$ (Ours)  & \textbf{97.0}$\pm$0.3 & \textbf{98.1}$\pm$0.5  & \textbf{98.3}$\pm$0.0 & \textbf{97.9}$\pm$0.1 & \textbf{98.4}$\pm$0.0 & {96.1}$\pm$0.1 & \textbf{96.9}$\pm$0.3 & \textbf{98.7}$\pm$0.5 & \textbf{95.4}$\pm$0.2  & \textbf{54.7}$\pm$3.8 &  \textbf{60.3}$\pm$2.0\\
    % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.2}& \textbf{78.4}  \\
    % \multicolumn{5}{c}{CARS} \\
    % \midrule
    % PIP-Net & 86.5 & 669 & 11  \\
    % ProtoPool & 88.9 & 195 & 195 \\
    \bottomrule
  \end{tabular}
  %}

\end{sidewaystable}
\begin{sidewaystable}[htbp]
%\resizebox{\linewidth}{!}{
  \caption{
  \accmetricstablestart{\gls{incv}}
  \boldnessstatement
  %Comparison on typical metrics for prototype-based methods with \gls{incv} as backbone: \gls{NewlayerName} shows increased accuracy with increased compactness. \boldnessstatement
  %The * indicates reported values which could not be reproduced.
  }
  \label{stab:incaCCproto-table}
  \centering
  \begin{tabular}{lccccccccc}
    \toprule
    Method &  \multicolumn{3}{c}{Accuracy \arrowUp} &
    \multicolumn{3}{c}{Total Features\arrowDown} & \multicolumn{3}{c}{Features / Class\arrowDown} \\
   & CUB& CARS & TRAVEL   & CUB& CARS & TRAVEL   & CUB& CARS &TRAVEL  
    \\
    \midrule
    Baseline  \gls{incv} & {86.1}$\pm$0.1 & {92.6}$\pm$0.2 & {68.7}$\pm$0.4 & 2048 & 2048 & 2048& 2048& 2048 &2048\\
    \midrule
    \glmtable{} & {79.2}$\pm$0.5 & {89.3}$\pm$0.3 & {63.4}$\pm$0.5  & 814$\pm$9 & 795$\pm$8 & 813$\pm$9 & \textbf{5}& \textbf{5} &\textbf{5} \\
    \slddtable{} & {83.1}$\pm$0.4 & {91.1}$\pm$0.2 & {69.9}$\pm$0.2  &  \textbf{50} & \textbf{50} &\textbf{50}& \textbf{5}& \textbf{5} &\textbf{5} \\
     \midrule
     \gls{NewlayerName} (Ours)  & \underline{84.2}$\pm$0.4 & \textbf{{91.7}}$\pm$0.1 & \textbf{71.5}$\pm$0.4 & \textbf{50} & \textbf{50} &\textbf{50}&  \textbf{5}& \textbf{5} &\textbf{5} \\ % Imgs, 74,192, 74.07, 74.254
   % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.3}& \textbf{77.2} & -&202 &195& 202&-& \textbf{5} &\textbf{5} &\textbf{5} &- \\
    $\gls{nperClass}=10$ (Ours)  & \textbf{84.4}$\pm$0.4 & \textbf{91.7}$\pm$0.2 & \underline{70.8}$\pm$0.3 &\textbf{50} &\textbf{50}& \textbf{50}& 10 &10 &10  \\
    % \multicolumn{5}{c}{CARS} \\
    % \midrule
    % PIP-Net & 86.5 & 669 & 11  \\
    % ProtoPool & 88.9 & 195 & 195 \\
    \bottomrule
  \end{tabular}
  %}

  
\end{sidewaystable}
\begin{sidewaystable}[htbp]
%\resizebox{\textwidth}{!}{
  \caption{
  \interpmetricstablestart{\gls{incv}}}
  %Comparison on Interpretability metrics with \gls{incv} as backbone. Due to required annotations, \cubsim{} can only be computed for \travelingheader{} and \cubheader{}. \boldnessstatement}
  \label{stab:incInterpproto-table}
  \centering
  \begin{tabular}{lccccccccccc}
    \toprule
    Method &  \multicolumn{3}{c}{\loc{5} \arrowUp} &
    \multicolumn{3}{c}{\generality{}\arrowUp} & \multicolumn{3}{c}{\contrastiveness{}\arrowUp} & \multicolumn{2}{c}{\cubsim{}\arrowUp} \\
  & CUB& CARS & TRAVEL   & CUB& CARS & TRAVEL   & CUB& CARS &TRAVEL   & CUB&TRAVEL
    \\
    \midrule
    Baseline  \gls{incv} & {38.9}$\pm$0.3 & {33.1}$\pm$0.2 & {40.7}$\pm$0.4  & {96.1}$\pm$0.0 & {95.7}$\pm$0.0 & {95.9}$\pm$0.0  & {89.6}$\pm$0.2 & {91.7}$\pm$0.2 & {89.8}$\pm$0.1& {7.1}$\pm$9.6 &  {24.1}$\pm$0.3 \\
    \midrule
    \glmtable{}  & {39.3}$\pm$0.2 & {34.0}$\pm$0.4 & {41.0}$\pm$0.3  & \underline{95.4}$\pm$0.0 & \underline{95.0}$\pm$0.0 & \underline{95.3}$\pm$0.0 & {91.3}$\pm$0.3 & {93.4}$\pm$0.2 & {91.2}$\pm$0.1 & {0.3}$\pm$0.4 &  {2.5}$\pm$2.8 \\
    \slddtable{}
     & \textbf{58.1}$\pm$1.2 & \textbf{52.1}$\pm$1.5 & \textbf{60.5}$\pm$1.3  & {92.6}$\pm$0.1 & {92.1}$\pm$0.1 & {92.6}$\pm$0.2 & \underline{93.0}$\pm$0.3 & \textbf{94.4}$\pm$0.2 & {92.3}$\pm$0.3 & {24.4}$\pm$2.3 &  {27.2}$\pm$5.2 \\
      \midrule
     \gls{NewlayerName} (Ours) & {48.6}$\pm$0.9 & {42.8}$\pm$0.8 & {50.2}$\pm$0.4 & {95.1}$\pm$0.1 & {94.7}$\pm$0.0 & {95.1}$\pm$0.1 & \textbf{93.4}$\pm$0.1 & \underline{94.3}$\pm$0.1 & \textbf{93.4}$\pm$0.1&  \underline{34.8}$\pm$3.4 &  \underline{44.3}$\pm$3.8 \\
     $\gls{nperClass}=10$ (Ours)  & \underline{54.6}$\pm$0.6 & \underline{47.1}$\pm$0.5 & \underline{55.0}$\pm$1.4  &   \textbf{96.9}$\pm$0.1 & \textbf{96.8}$\pm$0.0 & \textbf{96.9}$\pm$0.1  & {92.6}$\pm$0.2 & {93.6}$\pm$0.2 & \underline{92.6}$\pm$0.2  & \textbf{41.9}$\pm$3.0 &  \textbf{50.3}$\pm$1.6 \\
    % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.2}& \textbf{78.4}  \\
    % \multicolumn{5}{c}{CARS} \\
    % \midrule
    % PIP-Net & 86.5 & 669 & 11  \\
    % ProtoPool & 88.9 & 195 & 195 \\
    \bottomrule
  \end{tabular}
 % }

\end{sidewaystable}

% \begin{sidewaystable}[htbp]
% %\resizebox{\linewidth}{!}{
%   \caption{
%   \accmetricstablestart{Swin Transformer small}
%   \boldnessstatement
%   %Comparison on typical metrics for prototype-based methods with \gls{incv} as backbone: \gls{NewlayerName} shows increased accuracy with increased compactness. \boldnessstatement
%   %The * indicates reported values which could not be reproduced.
%   }
%   \label{sstab:incaCCproto-table}
%   \centering
%   \begin{tabular}{lccccccccc}
%     \toprule
%     Method &  \multicolumn{3}{c}{Accuracy \arrowUp} &
%     \multicolumn{3}{c}{Total Features\arrowDown} & \multicolumn{3}{c}{Features / Class\arrowDown} \\
%    & CUB& CARS & TRAVEL   & CUB& CARS & TRAVEL   & CUB& CARS &TRAVEL  
%     \\
%     \midrule
%     Baseline  Swin Transformer small & {87.0}$\pm$0.1 & {90.6}$\pm$0.6 & {59.0}$\pm$0.4  & 768 & 768 & 768& 768& 768 &768\\
%     \midrule
%     \glmtable{}  & {76.5}$\pm$0.4 & {75.5}$\pm$1.2 & {46.4}$\pm$1.0  & 572$\pm$4 & 559$\pm$8 & 561$\pm$11 & \textbf{5}& \textbf{5} &\textbf{5} \\
%     \slddtable{} &   \underline{85.3}$\pm$0.4  & \textbf{89.1}$\pm$0.7 & {60.3}$\pm$1.0 &  \textbf{50} & \textbf{50} &\textbf{50}& \textbf{5}& \textbf{5} &\textbf{5} \\
%      \midrule
%      \gls{NewlayerName} (Ours)   & {85.0}$\pm$0.4 & {88.7}$\pm$0.5 & \textbf{61.0}$\pm$1.0& \textbf{50} & \textbf{50} &\textbf{50}&  \textbf{5}& \textbf{5} &\textbf{5} \\ % Imgs, 74,192, 74.07, 74.254
%    % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.3}& \textbf{77.2} & -&202 &195& 202&-& \textbf{5} &\textbf{5} &\textbf{5} &- \\
%     $\gls{nperClass}=10$ (Ours)  &  \textbf{85.4}$\pm$0.3&  \underline{89.0}$\pm$0.8 & \underline{60.9}$\pm$1.1 &\textbf{50} &\textbf{50}& \textbf{50}& 10 &10 &10  \\
%     % \multicolumn{5}{c}{CARS} \\
%     % \midrule
%     % PIP-Net & 86.5 & 669 & 11  \\
%     % ProtoPool & 88.9 & 195 & 195 \\
%     \bottomrule
%   \end{tabular}
%   %}

  
% \end{sidewaystable}
% \begin{sidewaystable}[htbp]

%   \caption{
%   \interpmetricstablestart{Swin Transformer small}}
%   %Comparison on Interpretability metrics with \gls{incv} as backbone. Due to required annotations, \cubsim{} can only be computed for \travelingheader{} and \cubheader{}. \boldnessstatement}
%   \label{sstab:incInterpproto-table}
%   \resizebox{\textwidth}{!}{
%   \centering
%   \begin{tabular}{lccccccccccc}
%     \toprule
%     Method &  \multicolumn{3}{c}{\loc{5} \arrowUp} &
%     \multicolumn{3}{c}{\generality{}\arrowUp} & \multicolumn{3}{c}{\contrastiveness{}\arrowUp} & \multicolumn{2}{c}{\cubsim{}\arrowUp} \\
%   & CUB& CARS & TRAVEL   & CUB& CARS & TRAVEL   & CUB& CARS &TRAVEL   & CUB&TRAVEL
%     \\
%     \midrule
%     Baseline  Swin Transformer small  & {26.4}$\pm$0.1 & {26.0}$\pm$0.1 & {29.6}$\pm$0.2   & {96.8}$\pm$0.0 & f{96.6}$\pm$0.0 & {96.9}$\pm$0.1  & {98.3}$\pm$0.1 & {98.8}$\pm$0.1 & {97.4}$\pm$0.1 & {24.5}$\pm$0.4 & {23.6}$\pm$0.9 \\
%     \midrule
%     \glmtable{} & {26.4}$\pm$0.2 & {26.1}$\pm$0.1 & {30.0}$\pm$0.4 &  \underline{96.6}$\pm$0.0 & \underline{96.4}$\pm$0.0 & \underline{96.7}$\pm$0.0  & \textbf{99.1}$\pm$0.1 & \textbf{99.6}$\pm$0.0 & {98.3}$\pm$0.1  & {8.8}$\pm$2.8  & {6.9}$\pm$1.5 \\
%     \slddtable{}
%      & \underline{38.0}$\pm$0.5 & \underline{35.6}$\pm$1.1 & \underline{43.2}$\pm$1.4 & {93.4}$\pm$0.1 & {93.3}$\pm$0.2 & {93.6}$\pm$0.2  & \underline{99.0}$\pm$0.2 & \underline{99.4}$\pm$0.2 & \textbf{99.3}$\pm$0.4  & {37.2}$\pm$3.4 &  {40.6}$\pm$2.4\\
%       \midrule
%      \gls{NewlayerName} (Ours) & {33.6}$\pm$0.4 & {32.0}$\pm$0.3 & {37.9}$\pm$0.7  & {95.2}$\pm$0.0 & {94.7}$\pm$0.0 & {95.2}$\pm$0.1 &  {98.5}$\pm$0.3 & {99.1}$\pm$0.2 & \underline{99.1}$\pm$0.3   & \underline{45.1}$\pm$3.2 & \underline{43.1}$\pm$3.4 \\
%      $\gls{nperClass}=10$ (Ours)  & \textbf{40.4}$\pm$0.7 & \textbf{37.3}$\pm$1.7 & \textbf{44.6}$\pm$1.2  & \textbf{96.9}$\pm$0.0 & \textbf{96.6}$\pm$0.0 & \textbf{96.9}$\pm$0.1   & {95.5}$\pm$0.3 & {97.7}$\pm$0.6 & {94.7}$\pm$1.0  & \textbf{52.1}$\pm$2.1 & \textbf{52.5}$\pm$2.0 \\
%     % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.2}& \textbf{78.4}  \\
%     % \multicolumn{5}{c}{CARS} \\
%     % \midrule
%     % PIP-Net & 86.5 & 669 & 11  \\
%     % ProtoPool & 88.9 & 195 & 195 \\
%     \bottomrule
%   \end{tabular}
%  }

% \end{sidewaystable}

% \begin{sidewaystable}[htbp]

%   \caption{
%   \accmetricstablestart{Swin Transformer tiny}
%   \boldnessstatement
%   %Comparison on typical metrics for prototype-based methods with \gls{incv} as backbone: \gls{NewlayerName} shows increased accuracy with increased compactness. \boldnessstatement
%   %The * indicates reported values which could not be reproduced.
%   }
%   %\resizebox{\linewidth}{!}{
%   \label{tstab:incaCCproto-table}
%   \centering
%   \begin{tabular}{lccccccccc}
%     \toprule
%     Method &  \multicolumn{3}{c}{Accuracy \arrowUp} &
%     \multicolumn{3}{c}{Total Features\arrowDown} & \multicolumn{3}{c}{Features / Class\arrowDown} \\
%    & CUB& CARS & TRAVEL   & CUB& CARS & TRAVEL   & CUB& CARS &TRAVEL  
%     \\
%     \midrule
%     Baseline  Swin Transformer tiny & {86.6}$\pm$0.2 & {90.3}$\pm$0.3 & {60.1}$\pm$0.6 & 768 & 768 & 768& 768& 768 &768\\
%     \midrule
%     \glmtable{} & {71.8}$\pm$2.0 & {70.8}$\pm$1.4 & {46.6}$\pm$1.5  & 559$\pm$15 & 559$\pm$9 & 569$\pm$10 & \textbf{5}& \textbf{5} &\textbf{5} \\
%     \slddtable{} & {84.4}$\pm$0.3 & \textbf{88.4}$\pm$1.3 & {58.3}$\pm$0.7 &  \textbf{50} & \textbf{50} &\textbf{50}& \textbf{5}& \textbf{5} &\textbf{5} \\
%      \midrule
%      \gls{NewlayerName} (Ours)   & \underline{84.5}$\pm$0.4 & {88.0}$\pm$1.3 & \underline{59.3}$\pm$0.9  & \textbf{50} & \textbf{50} &\textbf{50}&  \textbf{5}& \textbf{5} &\textbf{5} \\ % Imgs, 74,192, 74.07, 74.254
%    % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.3}& \textbf{77.2} & -&202 &195& 202&-& \textbf{5} &\textbf{5} &\textbf{5} &- \\
%     $\gls{nperClass}=10$ (Ours)   & \textbf{84.6}$\pm$0.4 & \underline{88.3}$\pm$1.0 & \textbf{59.8}$\pm$0.9&\textbf{50} &\textbf{50}& \textbf{50}& 10 &10 &10  \\
%     % \multicolumn{5}{c}{CARS} \\
%     % \midrule
%     % PIP-Net & 86.5 & 669 & 11  \\
%     % ProtoPool & 88.9 & 195 & 195 \\
%     \bottomrule
%   \end{tabular}
% %  }

  
% \end{sidewaystable}
% \begin{sidewaystable}[htbp]
% %
%   \caption{
%   \interpmetricstablestart{Swin Transformer tiny}}
%   %Comparison on Interpretability metrics with \gls{incv} as backbone. Due to required annotations, \cubsim{} can only be computed for \travelingheader{} and \cubheader{}. \boldnessstatement}
%   \label{tstab:incInterpproto-table}
%   \resizebox{\textwidth}{!}{
%   \centering
%   \begin{tabular}{lccccccccccc}
%     \toprule
%     Method &  \multicolumn{3}{c}{\loc{5} \arrowUp} &
%     \multicolumn{3}{c}{\generality{}\arrowUp} & \multicolumn{3}{c}{\contrastiveness{}\arrowUp} & \multicolumn{2}{c}{\cubsim{}\arrowUp} \\
%   & CUB& CARS & TRAVEL   & CUB& CARS & TRAVEL   & CUB& CARS &TRAVEL   & CUB&TRAVEL
%     \\
%     \midrule
%     Baseline  Swin Transformer tiny  & {27.3}$\pm$0.2 & {26.3}$\pm$0.1 & {30.9}$\pm$0.2  & {96.8}$\pm$0.0 & {96.6}$\pm$0.0 & {96.9}$\pm$0.0 & {98.8}$\pm$0.0 & {99.0}$\pm$0.1 & {98.4}$\pm$0.1 & {26.1}$\pm$0.2 & {23.1}$\pm$0.4\\
%     \midrule
%     \glmtable{}   & {26.4}$\pm$0.2 & {25.9}$\pm$0.1 & {29.9}$\pm$0.3  & \underline{96.6}$\pm$0.0 & \textbf{96.5}$\pm$0.0 & \underline{96.7}$\pm$0.0& \textbf{99.3}$\pm$0.0 & \textbf{99.5}$\pm$0.1 & \textbf{98.9}$\pm$0.1  & {12.1}$\pm$3.9 & {6.1}$\pm$2.2 \\
%     \slddtable{}
%       & \underline{38.9}$\pm$0.6 & \underline{35.4}$\pm$1.6 & \underline{46.6}$\pm$0.7  & {93.3}$\pm$0.2 & {92.9}$\pm$0.1 & {93.6}$\pm$0.2 & \underline{99.2}$\pm$0.3 & \underline{99.3}$\pm$0.4 & \textbf{98.9}$\pm$0.2  & {43.8}$\pm$5.7 & {41.2}$\pm$1.4\\
%       \midrule
%      \gls{NewlayerName} (Ours)  & {36.9}$\pm$0.4 & {31.5}$\pm$1.4 & {41.8}$\pm$0.3 & {95.1}$\pm$0.1 & {94.6}$\pm$0.1 & {95.3}$\pm$0.1 & {98.2}$\pm$0.4 & {98.7}$\pm$0.4 & {98.4}$\pm$0.2& \underline{50.9}$\pm$4.9 & \underline{51.4}$\pm$2.1 \\
%      $\gls{nperClass}=10$ (Ours)   & \textbf{44.6}$\pm$0.5 & \textbf{37.5}$\pm$0.4 & \textbf{48.5}$\pm$0.9  & \textbf{96.9}$\pm$0.0 & \textbf{96.5}$\pm$0.0 & \textbf{97.0}$\pm$0.0  & {93.8}$\pm$0.2 & {97.4}$\pm$0.8 & {92.8}$\pm$0.7   & \textbf{54.7}$\pm$3.8 & \textbf{54.5}$\pm$2.6\\
%     % $\gls{nReducedFeatures}>50$ & \textbf{86.4} & \textbf{92.2}& \textbf{78.4}  \\
%     % \multicolumn{5}{c}{CARS} \\
%     % \midrule
%     % PIP-Net & 86.5 & 669 & 11  \\
%     % ProtoPool & 88.9 & 195 & 195 \\
%     \bottomrule
%   \end{tabular}
%   }

\end{sidewaystable}
